Personalized Adaptation via In-Context Preference Learning

Reinforcement Learning from Human Feedback (RLHF) is widely used to align Language Models (LMs) with human preferences. However, existing approaches often neglect individual user preferences, leading to suboptimal personalization. We present the Preference Pretrained Transformer (PPT), a novel approach for adaptive personalization using online user feedback. PPT leverages the in-context learning capabilities of transformers to dynamically adapt to individual preferences. Our approach consists of two phases: (1) an offline phase where we train a single policy model using a history-dependent loss function, and (2) an online phase where the model adapts to user preferences through in-context learning. We demonstrate PPT's effectiveness in a contextual bandit setting, showing that it achieves personalized adaptation superior to existing methods while significantly reducing the computational costs. Our results suggest the potential of in-context learning for scalable and efficient personalization in large language models.

==> 02_literature.tex <==
\section{Related Works}

\xhdr{LLM personalization}


\xhdr{RLHF with diverse preferences} Several approaches have been proposed to mitigate the issue of diverse preferences of different populations. A common strategy is to learn a reward model for each group of preferences and aggregate the reward models or learned policies, as in \citet{chakraborty2024maxminrlhfequitablealignmentlarge}, \citet{jang2023personalizedsoupspersonalizedlarge} and \citet{ramé2023rewardedsoupsparetooptimalalignment}. ...


\xhdr{In-context learning} Decision Pretrained Transformers (DPT) (\citet{lee2023supervisedpretraininglearnincontext}) are a recent advancement in reinforcement learning, where
the transformer predicts an optimal action given a query state and an in-context
dataset of interactions. ...

Our approach extends these ideas by introducing a history-dependent DPO, which minimizes the DPO loss at each turn of conversation such that the model is increasingly aligned with the user’s preferences as the conversation progresses.


==> 03_method.tex <==
\section{Pre-Training for Multi-Preference In-Context Adaptation}

Exact optimization of the objective function \cref{eq:optimal-model} can be challenging since the history (in-context data) $\history$ in the expectation also depends on the learnable model $M_\theta$. Here, we propose an approximation to this objective by replacing the distribution $\dist_{\cH} \lpar \cdot \midsem M_\theta, z^\star \rpar$ with the offline data $\data_\pre\href{}{}$. However, since we do not know the group identity $z^\star$, we optimize the summation over all the offline datasets:
\begin{align}
    \max_{M_\theta}\,  \sum_{i=1}^K \E_{x \sim \data, \history \sim \data^{(i)}_\pre, a \sim M_\theta \lpar x \midsem \history \rpar} \lbar r\lpar a \given x \midsem z^{(i)} \rpar \rbar  - \beta \kl{M_\theta\lpar x\midsem \history\rpar(a) }{\pi_{\text{ref}}\lpar a \given x \rpar}. \label{eq:approx-model}
\end{align}
Instead of learning a reward model and optimizing the above objective, we can follow a direct preference optimization (DPO) approach as in \citet{rafailov2023direct}. We can show optimizing the above objective is equivalent to miniziming the following loss function:
{\small
\begin{align}
    \loss\lpar M_\theta \midsem \pi_{\text{ref}} \rpar = - \sum_{j=1}^K \E_{\lcbar \lpar x, a, \bar{a} \rpar, H \rcbar \sim \data^{(i)}_\pre} \lbar \log \sigma \lpar \frac{\beta}{K} \log \frac{M_\theta\lpar x\midsem H \rpar(a)}{\pi_{\text{ref}}\lpar a \given x \rpar} + \frac{\beta}{K} \log \frac{\pi_{\text{ref}}\lpar \bar{a} \given x \rpar}{M_\theta\lpar x\midsem H \rpar(\bar{a})}\rpar \rbar.
\end{align}
}%
\vahidcomment{There is probably some link here between the fact the we're trying to keep $M_\theta$ similar to $\pi_{\text{ref}}$ in \cref{eq:optimal-model,eq:approx-model} and the fact that we're approximating the history coming from $M_\theta$ using the history from $\pi_{\text{ref}}$. We might be able to show the approximate objective in \cref{eq:approx-model} is close to the one in \cref{eq:optimal-model}.}



==> color-edits.tex <==
\ProvidesPackage{color-edits}

\def\@SuppressEdits{no}
\DeclareOption{suppress}{%
\def\@SuppressEdits{yes}
}

\def\@ShowDeletions{no}
\DeclareOption{showdeletions}{\def\@ShowDeletions{yes}}

\ProcessOptions

% Provides useful macros for making recent edits by different authors
% visible with colors in a jointly edited LaTeX document.
% Different authors are added with \addauthor{AUTH}{color}
% (the only exported command provided by this package).
% Invocation of \addauthor generates four new commands
% (where AUTH should be replaced by the supplied name of the author,
% e.g., initials, or whatever else is used):
% 1. \AUTHedit{text}: displayes the 'text' in the color assigned to the
% author.
% 2. \AUTHcomment{text}: generates '[AUTH: text]' in the color
% assigned, i.e., annotates the text as a comment written by the
% author.
% 3. \AUTHmargincomment{text}: generates a marker in the author's
% color at the given spot, and writes the text in the color in the
% margin. 
% 4. \AUTHdelete{text}: per default, displays a marker in the author's
% color at the given spot, and marks in the margin that the author
% deleted something in this place. (This allows co-authors to check
% what was deleted.)
%
% As an example, \addauthor{dk}{blue} generates the commands
% \dkedit{}, \dkcomment{}, \dkmargincomment{}, \dkdelete{}, all of
% which display material in blue.
%
% The package allows two options:
% 1. 'suppress' suppresses all comments and deletion markers, and
% removes the coloring from text in \AUTHedit{}. Thus, it essentially
% displays the text as it would be once all comments are explicitly
% removed (though there may be small spacing issues, so they should
% still be explicitly removed eventually).
% 2. 'showdeletions' replaces the semantics of the \AUTHdelete{text}
% command, so that instead the text is still displayed, but struck out
% (and in the color of the coresponding author). This allows
% co-authors to see more easily what has been deleted, without having
% to check the source code.

\usepackage{ifthen}
\usepackage{color}
\usepackage[normalem]{ulem}

\newcommand{\@edit}[2]{%
\ifthenelse{\equal{\@SuppressEdits}{yes}}{#2}{\textcolor{#1}{#2}}%
}

\newcommand{\@comment}[2]{%
\ifthenelse{\equal{\@SuppressEdits}{yes}}{}{\textcolor{#1}{#2}}%
}

\newcommand{\@margincomment}[2]{%
\ifthenelse{\equal{\@SuppressEdits}{yes}}{}{%
\textcolor{#1}{$[\bullet]$}%
\scriptsize\textcolor{#1}{#2}}%
}

\newcommand{\@delete}[3]{%
\ifthenelse{\equal{\@SuppressEdits}{yes}}{}{%
\ifthenelse{\equal{\@ShowDeletions}{yes}}{%
\textcolor{#1}{\sout{#2}}}{%
\textcolor{#1}{$[\bullet]$}%
\marginpar{\scriptsize\textcolor{#1}{#3 deleted here}}}}%
}

\newcommand{\addauthor}[2]{%
\expandafter\def\csname #1edit\endcsname ##1{\@edit{#2}{##1}}
\expandafter\def\csname #1comment\endcsname ##1{\@comment{#2}{[#1: ##1]}}
\expandafter\def\csname #1margincomment\endcsname ##1{\@margincomment{#2}{[#1: ##1]}}
\expandafter\def\csname #1delete\endcsname ##1{\@delete{#2}{##1}{#1}}
}



